Analysis of XLS-R for Speech Quality Assessment

In online conferencing applications, estimating the perceived quality of an audio signal is crucial to ensure high quality of experience for the end user. The most reliable way to assess the quality of a speech signal is through human judgments in the form of the mean opinion score (MOS) metric. However, such an approach is labor intensive and not feasible for large-scale applications. The focus has therefore shifted towards automated speech quality assessment through end-to-end training of deep neural networks. Recently, it was shown that leveraging pre-trained wav2vec-based XLS-R embeddings leads to state-of-the-art performance for the task of speech quality prediction. In this paper, we perform an in-depth analysis of the pre-trained model. First, we analyze the performance of embeddings extracted from each layer of XLS-R and also for each size of the model (300M, 1B, 2B parameters). Surprisingly, we find two optimal regions for feature extraction: one in the lower-level features and one in the high-level features. Next, we investigate the reason for the two distinct optima. We hypothesize that the lower-level features capture characteristics of noise and room acoustics, whereas the high-level features focus on speech content and intelligibility. To investigate this, we analyze the sensitivity of the MOS predictions with respect to different levels of corruption in each category. Afterwards, we try fusing the two optimal feature depths to determine if they contain complementary information for MOS prediction. Finally, we compare the performance of the proposed models and assess the generalizability of the models on unseen datasets.

==> revision-notes.tex <==
1. fixed capitalization of DNSMOS in reference [20]
2. fixed bold/underline in NISAQ column. Previously underlined XLS-R 1B Layer 41 (0.5657), but the minimum is actually XLS-R 1B Layer 10 (0.5456)
3. fixed mos visualization
- x/y labels were swapped
- dataset titles were swapped
- made spacing tighter to fit one more line of text on page
4. added human ACR visualization for IUB (and added sentence to figure caption)
5. no dropout in final model oops, but extra batchnorm after transformer apparently

% reviewers

